Using parametric set constraints for locating errors in CLP programs

This paper introduces a framework of parametric descriptive directional types for constraint logic programming (CLP). It proposes a method for locating type errors in CLP programs and presents a prototype debugging tool. The main technique used is checking correctness of programs w.r.t. type specifications. The approach is based on a generalization of known methods for proving correctness of logic programs to the case of parametric specifications. Set-constraint techniques are used for formulating and checking verification conditions for (parametric) polymorphic type specifications. The specifications are expressed in a parametric extension of the formalism of term grammars. The soundness of the method is proved and the prototype debugging tool supporting the proposed approach is illustrated on examples. The paper is a substantial extension of the previous work by the same authors concerning monomorphic directional types.

==> 33.tex <==






\subsection{Approximating program semantics}
\label{section.approx}

In this work we are mainly interested in checking program correctness.
However the representation of the verification condition (Proposition
\ref{ver.cond})
 as constraints (Lemma \ref{implication.as.constraints.lemma})
 can be used to obtain an approximation
of the semantics of a given program $P$. 
In the previous section we showed how a single implication from
Proposition \ref{ver.cond}
can be expressed by a constraint system $F_j(C)$.
We begin with constructing a constraint system representing all the
implications from the proposition.

Let us consider the constraints $F_j(C)$  ($j=1,\ldots,n_C$)
for each clause $C$ of $P$ with  $n_C$ body atoms.
Let  $F'_j(C)$ be  $F_j(C)$ with the variables renamed in
such a way that the only common variables of (distinct)
$F'_{j_1}(C_1)$, $F'_{j_2}(C_2)$ are $Call$ and  $Success$.
Let grammar $G_0$ specify the initial goals and the
constraint predicates.  So   \sem[G_0]{\Ca}\ is the set
of initial goals and of the allowed calls of constraints.
$\sem[G_0]{\Su}$
is (a superset of) the set of possible successes of constraint predicates.%
\footnote{
This approach can also be used when $P$ is a fragment of a program,
i.e.\ the clauses defining some predicates are missing in $P$.
Then the semantics of such predicates has to be specified by $G_0$.
The algorithm treats them as the constraint predicates.
Examples of such program fragments are programs using built-in predicates,
unfinished programs or modules of some bigger programs.
}
Thus $(\sem[G_0]\Ca, \sem[G_0]\Su)$ respects constraints.

Now any model $I$ of the constraint system
\[
{\cal C}(P) = \bigcup_{C\in P} \bigcup_j  F'_j(C) \ \cup\ G_0
\]
gives a specification
 $Spec=(I(\Ca),I(\Su))$
with respect to which $P$ is correct,
provided that $Spec$ respects constraints.
This follows immediately from Lemma \ref{implication.as.constraints.lemma}.

In the special case of logic programs a  model of ${\cal C}(P)$ can be
found by using the techniques for set constraint solving.
For example the technique of Heintze and Jaffar \shortcite{HJ90lics,HJ91}
produces 
a (non-discriminative) term grammar specifying the least model
of set constraints. This technique has been used for generating
approximations of logic program semantics %
\comment{PP:Dodaje HJ90popl i HJ94cpjak recenzent kazal.}
\cite{HJ90popl,Heintze92,HJ94cp,CP98}.
\comment{PP:uzupelniam nastepne zdanie o SAS97}
Another constraint solving approach that uses tree automata 
techniques, has been presented in 
\cite{DevienneTT97sas,TalbotDT2000}. 
We expect that these techniques can be generalized to the case
of CLP programs, but we did not investigate this
issue yet.
\comment{Bylo we wrzesniu
However, it has been pointed out by Heintze
that it is difficult to obtain acceptable efficiency of an
implementation of his constraint solving algorithms.
Therefore we leave the issue of generalizing the constraint solving
approaches as a topic of
future work and in our work we focus on another approach discussed below.
}
\comment{Poprzednie wersje i notatki

\comment{O cos nam tu chodzilo:\\
 In Section ... 
we sketch a rough  idea of such an extension.
\\
(czyli dolaczamy gdzie indziej - w rozdziale 4 ? sekcje
solving parametric constraints-
 cos w rodzaju zmodyfikowanej sekcji 3.1.3 gdzie wiezy  
 bez parametrow sa specjalnym przypadkiem ).
\\
Ale wyglada, ze tego nie zrobimy.

Nastepne zdanie trzeba wywazyc.
}
 However, it has been pointed out by Heintze
\cite{Heintze92}
\comment{ (tu dokladny cytat z podaniem strony)
that practical implementation
of his constraint solving algorithms may be rather difficult.

that the efficiency of practical implementations of his constraint
solving algorithms  is rather poor.
}
that it is difficult to obtain acceptable efficiency of an
implementation of his constraint solving algorithms.
This applies even more to the extension. Therefore we leave
the issue of implementation of the extension as a topic of
future work and in our work we focus on another approach discussed below.
}



Yet another approach to  finding a model of the constraint system 
${\cal C}(P)$  stems from abstract interpretation techniques
(among others \cite{JB92,HCC95}, \cite{GW94},
we generalize the latter work in
\cite{DrabentP99,DrabentMP99,DrabentMP00} and here). 
${\cal C}(P)$  is seen as a valuation transformer, its fixed points
are models of ${\cal C}(P)$.
Valuations are represented as discriminative grammars.
A fixed point is computed iteratively.  


To augment our system with a tool for computing approximations of program
semantics, we provide a
solution based on the latter idea.
This choice was guided mainly by possibility of reusing our
correctness checking algorithm
and the implementation of \cite{GW94}.


The correctness checking algorithm of the previous section can be
easily modified to compute the valuation transformer related to
${\cal C}(P)$.
This gives an implementation of a single step of
the iteration.  It remains to combine it with some technique of
assuring termination.

\medskip\noindent
\textbf{Iteration step.}
\
Take $G_i$ (initially $G_0$).
To each $ F'_j(C)  \cup G_i$ apply the construction as in the
correctness checking, obtaining a discriminative grammar $F_{C,j}$.
(It is required that all the obtained grammars have distinct variables,
except \Ca and \Su).
For each  $F_{C,j}$, the variables occurring in  $F_{C,j}$ are
distinct from those in $G_i$ except for \Ca or \Su.
\comment{
Nieprawda, ze: \ \ 
The least models of $ F'_j(C) \cup G_i$ and of
$F_{C,j}$ coincide on their common variables.
}

The constraints of  $F'_j(C)$ are satisfied if the occurrences of \Ca,
 \Su in the right hand side of each constraint of the form 
(\ref{implication.as.constraints1}) (Section \ref{section.ver.cond}) 
are valuated as in the least model
of $G_i$, and the remaining variable occurrences as in the least
model of  $F_{C,j}$.
This follows from the discussion in the previous section.
\comment{
   Mozna tez rozbic $F_{C,j}$ na czesci $G'$ i $G''$, jak w porzednim
   rozdziale,  i powiedziec, ze (1) sa spelnione w
   najmniejszym modelu  $G\cup G'$,  zas (2) w    $G'\cup G''$.
Ponizej, gdy mowimy o calym ${\cal C}(P)$, mozna to samo zrobic z  $G_{i+1}$.
}
\comment{
Chyba bez sensu: \\
Chyba wystarczy tylko $\gra[G_0]\Su$ zamiast $G_0$, ale to wymaga
dodatkowych wyjasnien.
}

The obtained grammar
 $G_i' = G_i\cup \bigcup_{C\in P} \bigcup_j  F_{C,j}$ is not discriminative,
due to the rules for \Ca and for \Su.
Construct a discriminative approximation of $G_i'$, more precisely a
discriminative grammar  $G_{i+1}$ such that
$\sem[G'_i]{\Ca}\subseteq\sem[G_{i+1}]{\Ca}$ and the same for \Su.
This is done by applying the union operation of
 Section~\ref{term-grammars}
to $G_i$ and all grammars $F_{C,j}$.
(So $G_{i+1}$ is
$G_i\mathop{\dot\cup} \dot{\bigcup}_{C\in P} \dot{\bigcup}_j  F_{C,j}$
with the variable $\Ca\dot\cup\ldots\dot\cup\Ca$ renamed into $\Ca$
and  $\Su\dot\cup\ldots\dot\cup\Su$ renamed into $\Su$.)
\comment{
To jest przyklad, jak pozornie potrzebna operacja zaokraglania do
discriminative grammars staje sie niepotrzebna
}

The obtained grammar $G_{i+1}$ has the following property.
${\cal C}(P) - G_0$ is true when  \Ca and \Su in
all the constraints of the form
(\ref{implication.as.constraints1}) (Section \ref{section.ver.cond}) 
are valuated as in the least model
of  $G_i$,
\Ca and \Su in the constraints of the form
(\ref{implication.as.constraints2}) (Section \ref{section.ver.cond})  
as in the least model of  $G_{i+1}$,
and the (renamed) variables of $P$ as in the least model of $G_i'$.
\comment{
Bylo: \ \ 
${\cal C}(P) - G_0$ is true when  \Ca and \Su in
all the constraints of the form
(\ref{implication.as.constraints1}) are valuated as in the least model
of  $G_i$
and all the other variable occurrences as in the least model of $G_i'$
(or in the least model of $G_{i+1}$).

I to w nawiasie jest nieprawda, w tej gramatyce nie wystepuja zmienne
z programu.  A chodzi nam o odniesienie do $G_{i+1}$.
}
\comment{
Bylo zle:
 ${\cal C}(P)$ is true when  \Ca and \Su in
(\ref{implication.as.constraints2}) are valuated as in the least model
of  $G_i'$ (or the least model of $G_{i+1}$)
and all the other variable occurrences as in the least model of $G_i$.
}
\comment{Another formulation, which is better?: \
There exists a ``solution'' of ${\cal C}(P)$ in which 
 \Ca and \Su in
(\ref{implication.as.constraints1}) are valuated as in the least model
\ldots
 and all the other variable occurrences as in \ldots
}

It remains to check whether the specification given by $G_{i+1}$
does not contain incorrect calls of constraint predicates.
  This boils down to checking whether 
all the calls of constraint predicates from the set
\sem[G_{i+1}]\Ca\ are also members of \sem[G_0]\Ca.
The latter is equivalent to
$\sem[F]\Ca\subseteq\sem[G_0]\Ca$,
where
$F = G_{i+1}-\{\,\Ca{>}A\mid A \mbox{ is not a constraint}\,\}$.
\comment{Mozna tez: \ \ 
$F = G_{i+1}-\{\,\Ca\mathop{>}p(\vec X)\mid
 p \mbox{ is not a constraint predicate}\,\}$.
}
Failure of the check means that we are unable to construct a
specification which respects constraints.  This suggests a program
error and an appropriate warning is issued.

This completes an iteration step.  Notice that the calls and successes
of constraint predicates
specified by $G_{i+1}$ are the same as those specified by $G_i$ and
thus by $G_0$ (induction on $i$).
For calls it follows from succeeding of the checks above.
For successes we have that
any clause $\Su\mathop>p(\vec X)$ from  $G_{i+1}$,
where $p$ is a constraint predicate,
occurs also in $G_i$.






The iteration is terminated if a fixpoint is reached, this means
when
$\sem[G_{i+1}]{\Ca} \subseteq \sem[G_i]{\Ca}$ and
$\sem[G_{i+1}]{\Su} \subseteq \sem[G_i]{\Su}$.
(The inclusion in the other direction holds for each $i$).
The required model of   ${\cal C}(P)$ is 
a valuation in which the values of the variables from $G_0$, except
for \Ca and \Su, are as in the least model of  $G_0$,
 the values of  \Ca, \Su are as in the least model of
$G_{i}$,
and the variables of $P$ are valuated by the least model of $G_i'$.
{\sloppy\par}

As a result we obtain that whenever the iteration terminates,
program $P$ is correct w.r.t.\ the
specification given by the obtained grammar $G_{i}$.

Notice that this is justified in a
different way than usually done in abstract interpretation.
Instead of relating a single iteration step to the concrete semantics
of the program, we showed that the obtained fixpoint satisfies  
a sufficient condition for program correctness.

\comment{Was: \ \ \
Such iterative techniques are usually justified without a reference to
set constraints or sufficient conditions for correctness.
Instead, the technique is seen as an instance of the abstract
interpretation paradigm.
The valuation transformer is shown to be correct w.r.t.\ a
function defining a fixpoint semantics of the program.  
Hence the fixpoint found approximates the program's semantics.
}



\medskip\noindent



\textbf{Termination.}
\
Usually the iterative process described above does not terminate.
It should be augmented with means of assuring termination.
The idea is to apply a {\em restriction} operator $\cal R$
that maps an infinite domain of grammars to its finite subset.
Moreover,
 the operator $\cal R$ 
computes an approximation of a grammar $G$ (i.e.\ $\sem[G]{\Ca} \subseteq \sem[{\cal R}(G)]{\Ca}$ and 
$\sem[G]{\Su} \subseteq \sem[{\cal R}(G)]{\Su}$).  
The operator is applied in every iteration step: the newly obtained
grammar $G_{i+1}$  
is replaced by a grammar  $H_{i+1} = {\cal R}(G_{i+1})$.
In this way we obtain a sequence of grammars $G_0, H_1, H_2, \ldots$,
the sequence has the properties described in the previous paragraphs.
Since the co-domain of $\cal R$ is finite, the set of grammars 
$\{\,G_0,  H_1, H_2, \ldots\,\}$ is finite and the iteration terminates.
This technique can be seen as an instance of widening
\cite{CousotJLP92}.

An attempt at such approach was made by Gallagher and de Waal  \shortcite{GW94}.
Unfortunately, the termination proof given by the authors is erroneous
and Mildner \shortcite{Mil99} showed an artificial example which
results in an infinite loop.





We adapt a technique
presented  in \cite{Mil99}, Section 6.5, and inspired by  \cite{JB92}.
We describe it briefly.
Let the {\em principal label} of a variable $X$ be the set of function symbols occurring in the 
right hand sides of the rules defining $X$ in a given grammar $G$. 
Let a {\em term grammar graph} be a directed graph with grammar  variables as vertices.
An edge $(X,Y)$ belongs to the graph iff there is a rule $X > f(\ldots,Y,\ldots)$ in the grammar.
The operator $\cal R$ 
computes an approximation of a grammar $G$ (\,$\sem[G]{\Ca} \subseteq \sem[{\cal R}(G)]{\Ca}$ and 
$\sem[G]{\Su} \subseteq \sem[{\cal R}(G)]{\Su}$) 
assuring at the same time that there is 
a spanning tree of the graph of ${\cal R}(G)$ such that
each branch of the tree contains no more than $k$
variables with the same principal label.
Since the grammar is discriminative, and
since there is a finite number of function symbols in a program,
the set of such spanning trees (modulo variable renaming), is finite
and consequently the co-domain of $\cal R$ (modulo variable
renaming) is finite.
We usually apply $k=1$.

 The reasoning above
 does not provide any useful estimation of
 the complexity of the algorithm.  Our experience shows that it is
 sufficiently efficient to compute directional types of
 medium size programs. 



There exist variants of this method, taking into account a number of occurrences of a 
single function symbol along a path or just simply binding a depth of the 
spanning tree with a constant.

Another possibility to cope with the termination problem is to restrict the class of grammars
so that the class of defined sets is a partial order 
of finite heights\footnote{For example Boye \shortcite{Boy96} suggested
that the inference is always done with a finite lattice of types.
In practice this means that for a class of applications we may 
have a finite library of types, represented by grammars, which
may be extended by need. This will also facilitate 
 communication with the user who will easier  understand standard
application-specific types than the types represented by automatically
generated grammars.}. 



















